BitGNN: Unleashing the Performance Potential of Binary Graph Neural Networks on GPUs

Recent studies have shown that Binary Graph Neural Networks (GNNs) are promising for saving computations of GNNs through binarized tensors. Prior work, however, mainly focused on algorithm designs or training techniques, leaving it open to how to materialize the performance potential on accelerator hardware fully. This work redesigns the binary GNN inference backend from the efficiency perspective. It fills the gap by proposing a series of abstractions and techniques to map binary GNNs and their computations best to fit the nature of bit manipulations on GPUs. Results on real-world graphs with GCNs, GraphSAGE, and GraphSAINT show that the proposed techniques outperform state-of-the-art binary GNN implementations by 8-22X with the same accuracy maintained. BitGNN code is publicly available.

==> algorithms/FinBoutBSpMM.tex <==
\begin{algorithm}[!ht]
\DontPrintSemicolon
\KwInput{AdjMat: RowPtr, ColInd, BitTiles, Tile-row ID $r$; InActMat;} 
\KwOutput{OutActMat$_{(b)}$}
$NT \gets $ RowPtr[$r$+1]-RowPtr[$r$]; $TS \gets \frac{SIMD\_unit}{tile\_dim}$

\For{each tile set $t_{s}$ where $s$ = 1 to $\lceil\frac{NT}{TS}\rceil$}
{
    \textbf{register} A $\gets$ BitTiles[$s$] for $s$ = 0 to $TS$-1
    
    \textbf{register} B $\gets$ InActMat[$k$] for $k$ = (ColInd[$s$]$\times$$tileDim$+\{0,1,2,...,$tileDim$-1\}) $\times$$hidden\_size$+($warpid\%W\times$32)+$laneid$ and $s$ = 0 to $TS$-1
    
    \textbf{register} a $\gets$ a $|$ \codefont{shfl(}A, $s$$\times$$tile\_dim$+$laneid$\codefont{)} $\ll$ (4$\times$($TS$-1-$s$)) for $s$ = 0 to $TS$-1 \tcp{do bit-concatenate}
    
    \For{$n$ = 0 to $tileDim$-1}
    {
        \If{((\codefont{shfl(}a,$n$\codefont{)} $\gg$ (31-k)) \& 0x1) for $k$ = 0 to $SIMD\_unit$-1}
        {
            c[$n$] $\gets$ c[$n$] + B[$k$]
        }
    } \tcp{compute bit-dot-product}
}
\textbf{register} rs[$n$] $\gets$ \codefont{brev(ballot(}c[$n$]$\geq$0\codefont{))} for $n$ = 0 to $tileDim$-1

OutActMat$_{(b)}$[$r$$\times$$tileDim$+$(warpid\%W)$$\times$$\#\_of\_nodes$+$n$] $\gets$ rs[$n$] for $n$ = 0 to $tileDim$-1

\caption{BSpMM.FBB}\label{alg-fbspmm}
\end{algorithm}


==> algorithms/FinFoutBSpMM.tex <==
\begin{algorithm}[!ht]
\DontPrintSemicolon
\KwInput{AdjMat: RowPtr, ColInd, BitTiles, Tile-row ID $r$; InActMat;} 
\KwOutput{OutActMat}
$NT \gets $ RowPtr[$r$+1]-RowPtr[$r$]; $TS \gets \frac{SIMD\_unit}{tile\_dim}$

\For{each tile set $t_{s}$ where $s$ = 1 to $\lceil\frac{NT}{TS}\rceil$}
{
    \textbf{register} A $\gets$ BitTiles[$s$] for $s$ = 0 to $TS$-1
    
    \textbf{register} B $\gets$ InActMat[$k$] for $k$ = (ColInd[$s$]$\times$$tileDim$+\{0,1,2,...,$tileDim$-1\}) $\times$$hidden\_size$+($warpid\%W\times$32)+$laneid$ and $s$ = 0 to $TS$-1
    
    \textbf{register} a $\gets$ a $|$ \codefont{shfl(}A, $s$$\times$$tile\_dim$+$laneid$\codefont{)} $\ll$ (4$\times$($TS$-1-$s$)) for $s$ = 0 to $TS$-1 \tcp{do bit-concatenate}
    
    \For{$n$ = 0 to $tileDim$-1}
    {
        \If{((\codefont{shfl(}a,$n$\codefont{)} $\gg$ (31-k)) \& 0x1) for $k$ = 0 to $SIMD\_unit$-1}
        {
            c[$n$] $\gets$ c[$n$] + B[$k$]
        }
    } \tcp{compute bit-dot-product}
}
\If{$(warpid\%W)$$\times$32+$laneid$ $<$ $hidden\_size$}
{
    OutActMat[$r$$\times$$tileDim$$\times$$hidden\_size$ +$n$$\times$$hidden\_size$ +$(warpid\%W)$$\times$32+$laneid$] $\gets$ c[$n$] for $n$ = 0 to $tileDim$-1
}

\caption{BSpMM.FBF}\label{alg-ffspmm}
\end{algorithm}
